Characterizing Location-based Mobile Tracking in Mobile Ad Networks

Mobile apps nowadays are often packaged with third-party ad libraries to monetize user data.

==> algorithm.tex <==

\begin{algorithm}[!t]
\scriptsize
%\SetAlgoLined
%\KwResult{PII leakage across different locations}
\textbf{INPUT:} Predefined PII list (according to Table~\ref{tab:PII}), Domain organization mapping list.\\
\textbf{OUTPUT:} PII leakage of each app
\begin{algorithmic}[1]
\For{\textbf{each} App}
\For {\textbf{each} location}
\State Extract Gets and Posts URLs from captured traffic flows
\State Extract key-value pairs from the URLs
\State Match the key-value pairs with hashed PII values in PII list
 \If {find a match}
   \State Log the key-value pair as a PII leakage for the app  
\State Extract domains associated with the key-value pair
\State Match domains to the domain organization mapping list
  \If {find a match}
   \State Log the key-value pair as a PII leakage for the matched organization
\Else
   \State Log the key-value pair as a PII leakage for ``Others" organization
\EndIf
   \EndIf
\EndFor
\EndFor
\State \textbf{Return} PII leakage results
\end{algorithmic}
 \caption{PII Leakage Identification Algorithm}
 \label{alg:algo1}
\end{algorithm}
